On signal strength-based distance estimation using UWB technology

Ultra-wideband (UWB) technology has become very popular for indoor positioning and distance estimation (DE) systems due to its decimeter-level accuracy achieved when using time-of-flight-based techniques. Techniques for DE relying on signal strength (DESS) received less attention. As a consequence, existing benchmarks consist of simple channel characterizations rather than methods aiming to increase accuracy. Further development in DESS may enable lower-cost transceivers to applications that can afford lower accuracies than those based on time-of-flight. Moreover, it is a fundamental building block used by a recently proposed approach that can enable security against cyberattacks on DE which could not be avoided using only time-of-flight-based techniques. In this paper, we evaluate the suitability of several machine-learning models trained in different real-world environments to increase UWB-based DESS accuracy. Additionally, aiming for implementation in commercial off-the-shelf (COTS) transceivers, we propose and evaluate an approach to resolve ambiguities comprising DESS in these devices. Our results show that the proposed DE approaches have sub-decimeter accuracy when testing the models in the same environment and positions in which they have been trained, and achieved an average MAE of 24 cm when tested in a different environment. 3 datasets obtained from our experiments are made publicly available.

==> sections/7-acknowledgments.tex <==
\section*{ACKNOWLEDGEMENTS}
\label{acknowledgments}

This research has been funded by the Austrian Research Promotion Agency (FFG) and the Austrian Federal Ministry for Transport, Innovation an  Technology (BMVIT), within  the "ICT of the Future" project IoT4CPS (Trustworthy IoT for Cyber-Physical Systems) (FFG, \#863129) and COMET Center Pro\textsuperscript{2}Future (FFG, \#881844) and has been partially supported by the TU Graz LEAD project Dependable Internet of Things. 

Additionally, we would like to thank Georgios	Koutroulis and Milot Gashi for their support reviewing the text. 



==> sections/7-conclusion.tex <==
%!TEX root = ../main.tex
\section{CONCLUSIONS AND FUTURE WORK}
\label{conclusions}
In this paper we investigated the use of \ac{ml} regressors for \ac{uwb} \ac{de} using only signal-strength-related features. Successive analyses enabled finding more suitable parameters, features and regressors to this end, as well as discarding approaches which do not lead to a higher accuracy. In the current state, the use of the proposed methods in high accuracy applications is encouraged only for fingerprinting.

Future work includes preprocessing the received signal, using different \ac{ml} models and tuning parameters of models already tested. We also believe that conducting more experiments, for instance, subject to obstructed \ac{los} between transceivers, would encourage and enable the search towards better methods in this direction.
